A FaaS File System for Serverless Computing

Serverless computing with cloud functions is quickly gaining adoption, but constrains programmers with its limited support for state management. We introduce a shared file system for cloud functions. It offers familiar POSIX semantics while taking advantage of distinctive aspects of cloud functions to achieve scalability and performance beyond what traditional shared file systems can offer. We take advantage of the function-grained fault tolerance model of cloud functions to proceed optimistically using local state, safe in the knowledge that we can restart if cache reads or lock activity cannot be reconciled upon commit. The boundaries of cloud functions provide implicit commit and rollback points, giving us the flexibility to use transaction processing techniques without changing the programming model or API. This allows a variety of stateful sever-based applications to benefit from the simplicity and scalability of serverless computing, often with little or no modification.

==> figs/fig-concurrency.tex <==
%!TEX root = ../faasfs.tex

\begin{figure}[!t]
  \centering
  \includegraphics[scale=1.0]{figs/concurrency.eps}
  \caption{\jss{Cut and focuson on TPC-C instead - get one thing working right} Success and abort rates for read-write workload exhibiting contention.}
  \label{fig:concurrency}
\end{figure}


==> tex/6_discussion.tex <==
%!TEX root = ../faasfs.tex

\section{Discussion}
\label{sec:discussion}

\subsection{Strict serializabilitiy vs. serializability}

Maintaining external (real-time) POSIX 

Access control in the cloud context is pretty different.
Also talk about this as future work.

Can reduce function startup times. PyWren reported difficulties

There is no way to partition the file system cache because there are no names for function instances

Is legacy code idempotent


==> tex/9_conclusion.tex <==
%!TEX root = ../faasfs.tex

\section{Conclusion}
\label{sec:conclusion}

We report on our experience developing \system, a transactional shared file system designed specifically to meet the needs of serverless applications.
Rather than relying on fragmented and provider-specific interfaces to storage, programmers now can use the familiar and ubiquitous POSIX file system API.

\system builds upon the original spirit of cloud functions, providing compatibility with existing software ecosystems while adding the benefits of autoscaling, pay-per-use, and a cloud provider-managed environment.
The design of \system relies heavily on two specific features of the cloud functions environment.
Cloud functions have finite execution duration, and their begin and end points give us an opportunity to introduce an optimistic implementation of transactions transparently, with no changes to the API or programming model.
Programmers are also accustomed to writing programs where cloud functions are the unit of fault tolerance.
The support for transactions in \system is consistent with this approach, and makes correctness easier to achieve.
Our evaluation shows that the performance of \system is usually comparable to that of traditional file systems, and that our POSIX implementation is sufficiently complete and compliant to run a variety of application benchmarks, as well as a full-stack web application.
We hope that \system will help open up serverless computing to a broader range of applications.


==> tex/x_cut.tex <==
\subsection{Data science}
\label{subsec:pysat}

We return to an early motivation for serverless research, drawing inspiration from PyWren~\cite{jonas2017occupy} which presented a vision of putting the power of the cloud into the hands of the many.
PyWren introduced a serverless \textit{map} operator for the cloud, which takes Python function, perhaps one from a script running on a laptop, and executes it in a cloud context.

Python has good libraries for marshalling objects, including functions, for transport between processes, however these have a built-in assumption that the receiving Python interpreter has access to the same modules and libraries as the sending one.
To overcome this problem PyWren includes tools for packaging an environment, saving it to cloud object storage, and loading it onto a cloud function at startup.
This is inefficient because it may transfers many unused dependencies.
It is also cumbersome because users must often manually prune their environments to bring them under the 512~MB limit of the AWS Lambda \texttt{/tmp} file system.

Clearly this use case calls for a shared file system.
In this demonstration, we took an example~\cite{seasonaloccurrence} provided with the Python Satellite Data Analysis Toolkit (pysat), an off-the-shelf data science tool, and modified it to use Python's built-in \texttt{multiprocessing} library.
This allows the program to execute in parallel, using a \texttt{map} operation to take advantage of multiple cores on one server.
We then wrote an API compatible variant of Python multiprocessing, \texttt{lambdamultiprocessing} which uses AWS Lambda instead of local processes.
Provided all necessary libraries are located on a \system mount, a one-line change to the \texttt{import} statement is all that is needed to switch to cloud-based execution (See listing~\ref{listing:program} \jss{put a box with pseudocode, including showing the line that we changed }.

\jss{TODO: fill results}
For this workload, the virtual environment is X1 MB and contains Y1 files.
During execution each worker loads X1 MB and Y1 files.
We ran an analysis of XXXX over YYYY weeks of data.
On the 8-core server under the desk this takes XX hours.
Using \system and AWS Lambda it takes YY minutes.
\jss{say something about fault tolerance}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Concurrency and Consistency}
\label{subsec:concurrency}

\jss{I think we will cut this experiment because we don't have time to get it right.}
A key promise of \system is to maintain the strong consistency guarantees provided by POSIX, which is important for running existing applications unmodified.
Equally important for compatibility, is achieving good performance.

In this workload each client reads first identifies a read block and a write block.
It issues POSIX byte-range locks on each of them, a shared lock for the read, and an exclusive lock for the write operation. It then reads, writes, and releases locks.
In the \system case it also wraps the entire sequence in a transaction.
It then sleeps for 10~ms before repeating the process.
We use a file size of 1~MB and a block size of 1 KB.
We choose read and write blocks at random, selecting from a ``hot block'' set comprising 20 blocks 20\% of the time, and from the rest of the file 80\% of the time.
We implement this experiment using EC2 instances to support comparison with NFS.

Figure~\ref{fig:concurrency} compares NFS and three alternative implementations of \system.
We note that \system elides locks, and relies on strict serializability of transactions to meet the POSIX linearizability guarantee.

NFS does not encounter any aborts, and reaches a maximum of 140~ops/s with 16 clients.
Performance declines and at 192 clients the server becomes unstable and quickly crashes.
The three implementations of \system that we evaluate differ in how they track changes at the server.
The ``File Versioned'' approach maintains a single timestamp for each file, whereas the ``Block Versioned'' approach associates a timestamp with each block in the file.
``Block Multiversioned'' not only tracks a version for each block of the file, but also maintains multiple versions at the server and allows clients to read past versions of a file.

The File Versioned implementation of \system doesn't do much better than NFS, achieving a maximum of 2,050~ops/s with 128 clients and declining after that, as aborts on commit rise.
It suffers from a high degree of false sharing because it tracks changes at a coarse granularity.
The Block Versioned implementation does better in this regard, and benefits from a form of multiversioning since client caches may contain versions different from the latest at the server. This implementation shows near-linear scalability up to 500 clients, reaching an success rate of over 40,000 transactions per second with an abort rate of 6\%.

Our Block Multiversioned implementation uses an undo log to deliver multiversioned reads from the server.
So long as they complete quickly enough (before the undo space becomes exhausted), read-only transactions will always succeed, and do so without waiting on writers.
For this experiment the feature turns out to be a disadvantage relative to the Block Versioned implementation, in which failing to read an older version results in a helpful early abort.


\input{figs/fig-concurrency}

\section{something}
Outside of the cloud, file system APIs represent a near-universal storage abstraction.
Programmers may use file systems directly from their own code, through libraries (as is common for images and videos, JSON, CSV, and other serialized data), or as substrates under databases.
File system APIs have retained their relevance even as storage hardware evolved across orders of magnitude of capacity and performance.
For many years, shared file systems played a central role in corporate and campus computing, and they continue to play an important one.
In the cloud, however, file systems have a mostly server-local and rather peripheral role---important data lives elsewhere.

\textbf{Idempotence}
Idempotence is a central part of the execution model for cloud functions.
The cloud functions runtime promises to execute a function submitted to a queue at least once, but it may do so more than once, possibly concurrently.

\system can make it easier to write idempotent applications.
The basic approach is to associate a UUID with each invocation request.
After beginning a transaction, first check to see whether the UUID exists already in the set of completed transactions (e.g., look for existence of a marker file).
If so then abort, if not add it and continue with the rest of the transaction.

\system takes advantage of idempotence in an important way.
Idempotence means that we are ready for optimistic execution.
This is the key to going fast in a distributed system.

\textbf{Aren't transactions slow?}
We conducted simulation studies of \system.
To keep our exploration simple we modeled network latency as the sole source of delay in the system.
Network throughput and compute are taken to be unbounded.

We compared linearizable atomic operations (including file system locks), blocking transactions, and optimistic transactions.

Need to have something to say about locality
We don't do fake restarts, we have real restarts
Don't support lock upgrades, abort in this case
Deadlock detection is performed each time a transaction blocks
The transaction trying to acquire the lock is killed
our model does not include failure
+ try - kill the youngest transaction
+ try a model where we do not wait to start (must keep track of all of the versions)
+ try an optimistic model where we don't have read/write timestamps but instead validate the reads and with an attached clock

Think time to complete a unit of work
Network transfer time



What transaction give us
- optimistic / speculative execution
- optimistic execution without transactions doesn't work well, e.g., take whatever we have at the start and go with it

Can we have optimistic execution of code with locks without transactions, or are they the same thing?

What are the relevant characteristics of the workload?
- How much internal delay is there - "think time" between data accesses
- How much locality is there? - average interval for which a client has exclusive access
- How much contention is there? - probability of more than one access to a block in a give time interval from a single node
- number accessing a block during a particular time window

Locality and contention really are the same thing, they refer to different parts of the curve on the 
self-other correlation time for joint access to a block

Fundamental time unit is network delay, but we build the picture without
network delay, so accesses are just surfaces and think time sits in between.
Think of a cube with axes (x: client, y:data, z:time)
locality means we have a surface facing us,
    less locality means some fragments of secondary surfaces
contention means that we have many clients accessing the data simultaneously - we do this by creating hot blocks

contention is the average density along the z axis, projected down

- replace superluminal with highly partitioned + delegation

What is the relationship between isolation and concurrency? Could we build a system that was concurrent and not isolated?

\jss{The following content is old}

\jss{Say something about access time updates}
\jss{Say something about overlay file systems}
While databases can offer various isolation and consistency guarantees, we note that \textit{strict serializability} is sufficient to ensure linearizability, as required by POSIX.
Strict serializability is a property stronger than \textit{serializability}.
Not only must the observed result of an execution correspond to some ordering of the transactions, it must also respect the real-time property (also known as external consistency). This is equivalent to linearizability among the units of atomicity, in this case the transactions, as applied to the database as a whole.


In practice, however, modern implementations such as Spanner~\cite{corbett2013spanner} and CockroachDB~\cite{cockroachdb} provide good performance to many workloads while ensuring strict serializability among distributed transactions at global scale, in the latter case without using any kind of specialized hardware.
We note that the overheads involved with cloud function invocation are typically on the order tens of milliseconds~\cite{wang2018peeking}, which gives us additional comfort in using transactional techniques since we know that their overheads are modest in comparison.

The research challenge in \system is to maintain strict serializability while also providing effective a highly effective client-side caching for performance.
We choose to use Optimistic Concurrency Control (OCC)~\cite{kung1981optimistic} implemented with timestamp-order~\cite{bernstein1981concurrency}.
This allows us to defer consistency checks so that they do not hold up execution.
While the benefit of this approach is speed, the drawback is wasted work, as OCC transactions must restart when conflicts occur, whereas with pessimistic approaches based on locking they can instead wait.
It also may be impossible impossible to guarantee progress under OCC~\cite{gray1992transaction}.
However, OCC continues to gain traction in modern high-performance database systems, and it seems that in practice its shortcoming can be mitigated~\cite{diaconu2013hekaton}.
In this context we are comfortable committing \system to the OCC approach.

We also note that OCC presents a particularly nice match to the characteristics of cloud functions.
At least-once-execution, discussed in Section~\ref{subsec:lambdaenv} means that programmers already strive to cloud functions that are \textit{idempotent}, meaning that executing them more than once is equivalent to executing them just once.
Ensuring that code is idempotent can be challenging, and but it means that programmers have already thought about the side effects of their functions, e.g., what happens when an API calls is made more than once.
Transactions as provided by \system can help make writing idempotent cloud functions easier, since the changes to the file system can commit atomically with a marker than indicates completion of specific unit of work.
Extensions such as distributed transactions, discussed along with others in Section~\ref{sec:futurework}, could make it even easier for programmer to write idempotent cloud functions, and to ensure correctness of their applications.

\begin{itemize}
\item \textit{AWS S3}. Objects live in a hierarchical namespace, as in a file system, but the similarities end here.
Whereas file system objects are mutable, and in POSIX require strong consistency (a linearizability guarantee, see Sec~\ref{subsec:posix}), S3 stores versioned immutable objects, and maintains a weak consistency model.
It's performance and cost characteristics also favor throughput-oriented workloads over iop-intensive workloads~\cite{jonas2019cloud}.
\item \textit{AWS DynamoDB}. Key-value storage provides an alternative to object storage, offering lower latency and a broader range of consistency models.
DyanmoDB inherits the eventual consistency model its predecessor Dynamo~\cite{decandia2007dynamo}, and adds strong consistency (linearizability) as an option, as well as support for multi-object transactions.
Values remain versioned and immutable, and it does not support partial object updates as is possible with a write to a file system.
DynamoDB Accelerator (DAX) is a caching layer that may be deployed between DynamoDB and the application, e.g., code in AWS Lambda.
While this can provide latency and cost savings, it still requires a network round-trip for each operation.
It also restricts applications to using DynamoDB's eventual consistency modes.
\end{itemize}
